A Multihorizon Approach for the Reliability Oriented Network Restructuring Problem, Considering Learning Effects, Construction Time, and Cables Maintenance Costs

This paper presents a techno-economic optimisation tool to study how the power system expansion decisions can be taken in a more economical and efficient way, by minimising the consequent costs of network reinforcement and reconfiguration. Analyses are performed to investigate how the network reinforcement and reconfiguration should be planned, within a time horizon of several years, by continuously keeping the network feasibility and ability to satisfy the load. The main contribution of this study is the inclusion of key features within the mathematical model to enhance the investment decision making process. A representative maintenance cost of existing cables and apparatus is included, to analyse the influence of the historical performance of the electric items on the investment decisions. A multihorizon methodology is developed to take into account the long term variation of the demand, combined with the long term variation of cables maintenance costs. Moreover, technological learning coefficients are considered, to take into account the investment costs reductions that arise when an investment in network restructuring and/or reconfiguration is repeated throughout the years. Finally, construction time constraints are included to find a proper investment scheduling that allows a feasible power flow, also during the years required to build a new connection or restructure an existing one. This study is also providing recommendations for future research directions within the power system reliability field. The analyses show the important and urgent need of proper methodologies for a better definition of cables projected maintenance costs and learning coefficients dedicated to network restructuring, reconfiguration and expansion.

==> Figures/maintenance.tex <==
\begin{figure}[!htbp] 
\centering
  \subfigure[multi-horizon decision making]{% 
    \resizebox{12cm}{2cm}{%
    \hspace{1.4cm}
    \begin{tikzpicture}
    [
    triangle/.style = {fill=blue!20, regular polygon, regular polygon sides=3 },
    node rotated/.style = {rotate=180},
    border rotated/.style = {shape border rotate=180}
    ]
    \draw[-] (1,0) -- (9,0) node [below] {};
    \draw[->] (8,0) -- (9.5,0) node [above] {$\mathcal{T}$ (Years)};
    \node[triangle, border rotated, fill=green!40!white] at (3,0) {};
    \node[triangle, border rotated, fill=cyan!40!white] at (6,0) {};
    \draw [decorate,decoration={brace,amplitude=10pt}]
    (3,0.2) -- (6,0.2) node [black,midway,above=0.3cm] { construction time};
    \foreach \x in {1,...,9}
    \draw (\x, 0.1) -- (\x, -0.1) node [below] [yshift=-3pt] {\x};
    \draw[fill=green!40!white] (1,-1) circle (0.1cm) node[right] [xshift=3pt] {new installation decision taken};
    \draw[fill=cyan!40!white] (6.5,-1) circle (0.1cm) node[right] [xshift=3pt] {new connection ready};
    \end{tikzpicture}
  } }
  \subfigure[forecast of cable costs]{% 
  \resizebox{12cm}{10cm}{%
    \begin{tikzpicture}
    \begin{axis}[
        width=\linewidth, % Scale the plot to \linewidth
        grid=major, % Display a grid
        grid style={dashed,gray!30}, % Set the style
        xlabel= $\mathcal{T}$ (Years), % Set the labels
        ylabel= Cost multipliers,
        legend pos=north west,
        x tick label style={rotate=90,anchor=east} % Display labels sideways
        ]
        % add a plot from table; you select the columns by using the actual name in
        % the .csv file (on top)
        \addplot  table [x=a, y=b, col sep=comma] {data.csv};
%       \addplot [only marks] table [x=c, y=d, col sep=comma] {data1.csv};
        \addlegendentry{cable maintenance cost}
        \addlegendentry{linear fit}
        \end{axis}
    \end{tikzpicture}
    } }
\caption{Example of a multi-horizon structure of the model. When a new installation decision is taken, the power flow will not be allowed throughout the construction time (see section $a$). The maintenance cost of the existing apparatus is supposed to increase over time (see section $b$)} 
\label{Fig-multihor}
\end{figure}
